Action Assembly: Sparse Imitation Learning for Text Based Games with Combinatorial Action Spaces

We propose a computationally efficient algorithm that combines compressed sensing with imitation learning to solve text-based games with combinatorial action spaces. Specifically, we introduce a new compressed sensing algorithm, named IK-OMP, which can be seen as an extension to the Orthogonal Matching Pursuit (OMP). We incorporate IK-OMP into a supervised imitation learning setting and show that the combined approach (Sparse Imitation Learning, Sparse-IL) solves the entire text-based game of Zork1 with an action space of approximately 10 million actions given both perfect and noisy demonstrations.

==> old_intro.tex <==
%Old abstract
    %We propose a computationally efficient algorithm for Imitation Learning in Markov Decision Processes with a natural language action space. Such action spaces are combinatorial in the size of the dictionary and practically consist of millions of actions. Our approach uses compressed sensing algorithms to find the words that compose an action from the sum of their embeddings. Simulations on the text-based game Zork show that our algorithm solves the entire game using imperfect demonstrations.


%\begin{quote}
%``West of House\\
%You are standing in an open field west of a white house, with a boarded front door.\\
%There is a small mailbox here."\\
%\strut$\enspace\enspace$\textit{- Zork 1, opening scene}
%\end{quote}

%\textbf{Quote alternative:}
%\begin{quote}
%``A priest, a rabbi, and a minister walk into a bar. The bartender slowly cracks a smile, opens his mouth to speak, but can’t find the words. Slowly he cracks a smile, looks around and says `So many jokes to choose from...' ''
%\end{quote}

% \begin{abstract}
%     %\del{We propose the first computationally efficient deep reinforcement learning algorithm for MDPs with combinatorial action spaces (e.g. text-based games).}
%     %\dis{I think we should capture the niche of text-based games. So I would say}\add{ "We propose a computationally efficient deep reinforcement learning algorithm for MDPs with combinatiorial action spaces. While this is a general method that can be applied to many domains, we focus specifically on text-based games."}%For example, in text-based RL problems, the action space can be all the sentences composed of words from a dictionary of size $d,$ i.e., $|A| = d^l,$ where $l$ is the size of the sentence. 
%     %\dis{The section below is not clear. I would remove the following:} \del{
%     %Our approach builds on the deep deterministic policy gradient (DDPG) algorithm, that differentiates the actor with respect to the critic, and avoids taking a max operation over the entire action space. After the actor outputs a continuous action, we search for the $k<<|A|$ nearest discrete actions in the action set, and select the maximal action among them using the critic. Under some assumptions on the dictionary (e.g. coherence), sparse reconstruction algorithms perform computationally efficient search (polynomial time) instead of considering all actions (exponential time).}
%     %\add{Our approach combines Deep Deterministic Policy Gradient (DDPG) with Orthogonal Matching Pursuit, a sparse reconstruction algorithm, to perform a computationally efficient search across the action space in polynomial time rather than exponential time.}
%     %\del{Specifically, our algorithm combines DDPG with Orthogonal Matching Pursuit}
%     %\add{Specifically, our algorithm attempts} to find a sparse combination of words, such that the sum of their embeddings is closest to the output of the actor. Simulations on the text-based game Zork show promising results.
%     We propose a computationally efficient deep reinforcement learning algorithm for MDPs with combinatiorial action spaces. %For example, in text-based RL problems, the action space can be all the sentences composed of words from a dictionary of size $d,$ i.e., $|A| = d^l,$ where $l$ is the size of the sentence. 
%     %\dis{The section below is not clear. I would remove the following:} \del{
%     %Our approach builds on the deep deterministic policy gradient (DDPG) algorithm, that differentiates the actor with respect to the critic, and avoids taking a max operation over the entire action space. After the actor outputs a continuous action, we search for the $k<<|A|$ nearest discrete actions in the action set, and select the maximal action among them using the critic. Under some assumptions on the dictionary (e.g. coherence), sparse reconstruction algorithms perform computationally efficient search (polynomial time) instead of considering all actions (exponential time).}
%     Our approach combines Deep Deterministic Policy Gradient (DDPG) with Orthogonal Matching Pursuit, a sparse reconstruction algorithm, to perform a computationally efficient search across the action space in polynomial time rather than exponential time.
%     %\del{Specifically, our algorithm combines DDPG with Orthogonal Matching Pursuit}
%     Specifically, our algorithm attempts to find a sparse combination of words, such that the sum of their embeddings is closest to the output of the actor. Simulations on the text-based game Zork show promising results.
% \end{abstract}

\section{Introduction}

\todo[inline]{Tom: move from RL ro IL}

While we might chuckle at a story like this, there is more here than just a joke. If we look carefully at what happened, we notice that the bartender of our story stumbled on his words \cite{aat_doug}, while thinking about how to start the joke. Such cognitive-behavior breakdowns often occur when there are many actions to choose from, as described in the Action-Assembly Theory (AAT, \citet{aat}). According to Greene, behaviour is described by two essential processes: representation and processing. Representation refers to the way information is coded and stored in the mind, whereas processing refers to the mental operations performed to retrieve this information \cite{greene2008action}. Having good representations of information and an efficient processing procedure allows us to quickly exploit highly rewarding nuances of an environment upon first discovery. 

%}On the other hand, solving decision making problems computationally must involve exploration of all action interactions. This is specifically challenging in problems with combinatorial action spaces, like
However, learning good representations and developing efficient action selection procedures is a major computational challenge for artificially intelligent agents that aim to solve sequential decision making problems. This is especially problematic when dealing with combinatorial action spaces, since the agent needs to explore all possible action interactions. Combinatorial action spaces are prevalent in many domains including natural language generation \citep{ranzato2015sequence,bahdanau2016actor}, finance \citep{moody2001learning,hull2003options,heaton2017deep}, industry 4.0 (e.g., IoT) \citep{preuveneers2017intelligent}, electric grids \citep{wen2015optimal} and more. For example, in text-based games \citep{cote2018textworld}, given a dictionary with $d$ entries (words), the number of possible sentences of length $l$ is $d^l$ (i.e., the size of the combinatorial action space).

%In sparse recovery the goal is to recover a sparse vector $x$ (e.g., a Bag-of-Words vector) given a sum of dictionary embeddings. Formally, the goal is to solve $\min ||x||_0$ $\text{s.t.} \enspace Dx = v$ where $D$ is a known dictionary and $v$ is the observed dense vector.





%In the game of Zork, the player is greeted with the above message and responds in free-text. While the game understands simple responses such as ``go north" and ``place sword in chest", it also understands complex commands such as ``put the lamp and sword in the case", ``look under the rug" and ``drop all except lantern". Text-based games \citep{cote2018textworld} are an example of one problem among many, in which a reinforcement learning algorithm must be able to cope with combinatorial action spaces - the number of possible commands is exponential in the dictionary size and each action is a combination of basic elements (words).

% Real world examples of why this is interesting

% Approaches which attempt to solve this
Previous approaches have tackled the problem of large action spaces with varying success \citep{dulac2015deep,he2016deep,zahavy2018learn}, however, none have specifically considered combinatorial action spaces and thus computational efficiency remains an open problem: (i) \citet{dulac2015deep} extends the Deep Deterministic Policy Gradients (DDPG - \citep{lillicrap2015continuous}) architecture to cope with discrete actions, yet their nearest neighbour approach requires comparing with the entire action set - $\bigO(|A|)$ comparisons; (ii) \citet{he2016deep} present the Deep Reinforcement Relevance Network (DRRN) architecture, which requires each action to be evaluated by the network, which results in a total of $\bigO(|A|)$ forward passes; (iii) \citet{zahavy2018learn}, Action-Elimination Deep Q Network (AE-DQN), considers a scenario in which there are many \textit{invalid} actions; it utilizes an elimination signal provided by the environment to learn which actions may be \textit{eliminated}, thus reducing the effective number of actions. Since this is a Q-learning approach, the output layer contains $|A|$ neurons, and the final projection layer performs $\bigO(|A|)$ operations. 

%We emphasize here that the lower bounds for learning in general MDPs (e.g. Q-learning \citep{sutton1998reinforcement}) still apply in our scenario, and each state-action pair has to be visited infinitely often in order to compute an optimal policy.
%\dis{Not sure why you need the following lines: Maybe place this later in the text?}\del{We emphasize here that the lower bounds for learning in general MDPs (e.g. UCRL \citep{jaksch2010near} and R-max \citep{brafman2002r}) still apply in our scenario, and each state-action pair has to be visited multiple times (in the worst case scenario) to compute an optimal policy. Nevertheless,}
Clearly, these approaches do not scale to combinatorial action spaces due to computational inefficiency. In particular, all previous works ignored the underlying action structure - each action is a composition of basic building blocks.

In this work we propose the first computationally efficient reinforcement learning (RL) algorithm for solving problems with combinatorial action spaces. Motivated by AAT, our algorithm learns a model of the world that allows it to efficiently search for optimal actions. Specifically our agent (Figure \ref{fig:algorithm}) is composed of a: 
%\dis{Do you not want an 'Agent Model'? A world model still seems unclear to me.} 
%\textbf{(1) World Model} - We train an encoder and an evaluator. The encoder generates continuous actions (a dense representation) and the evaluator is used to evaluate these actions. More specifically; our evaluator, similar to the critic in \citet{dulac2015deep}, learns the $Q$ value for each state-action pair. 
\textbf{(1) Encoder} - We train an encoder which generates continuous actions (a dense representation of the action).
\textbf{(2) Representation} - We represent words using embeddings, previously trained on a large corpus of text. \textbf{(3) Retrieval Mechanism} - Recently, \citet{arora2018compressed} demonstrated sparse reconstruction \cite{elad2010book} of documents from the sum of common embedding schemes such as Word2vec \citep{mikolov2013efficient} and GloVe \citep{pennington2014glove}. Given a continuous vector $\aae$, a sum of word embeddings, the goal of sparse reconstruction is to recover the Bag-of-Words (BoW) vector (a discrete vector representing the indices of the words from the dictionary which compose $\aae$). Similarly, we propose to reconstruct discrete actions, composed of words, from the continuous output of the encoder. The benefit of our approach is that, there exist \textit{computationally efficient algorithms} for sparse reconstruction, which under some assumptions on the structure of the dictionary (e.g., coherence - Definition \ref{def:coherence}) ensure perfect recovery of the sparse representation.


Figure \ref{fig:algorithm} presents an overview of our architecture called Encoder EVALuator SENSing nEtwork (EVAL-SENSE). This architecture comprises three distinct components, an Encoder, Evaluator - collectively the \textit{World Model} (Section \ref{ref:encoderevaluator}) and Sparse Reconstruction algorithm - the \textit{retrieval mechanism} (Section \ref{sec:k-omp}). As seen in the figure, the encoder receives a state (in the NLP setting, this compromises a sentence detailing the current state of the game) and computes a sum of word embeddings. Using our novel sparse reconstruction algorithm K-OMP (see Section \ref{sec:k-omp}), we provide K candidate Bag of Words (BoW) vectors which are fed into the evaluator. The evaluator computes an expected value for each action candidate and the action with the highest value is fed into a language model to yield a sentence that can be parsed by the game.  



%In this work we propose the first computationally efficient reinforcement learning (RL) algorithm for solving problems with combinatorial action spaces. Motivated by AAT, our algorithm learns a model of the world that allows it to efficiently search for optimal actions. Specifically our agent (Figure \ref{fig:algorithm}) is composed of a: \dis{Do you not want an 'Agent Model'? A world model still seems unclear to me.} \textbf{(1) World Model} - We train an encoder and an evaluator. The encoder generates continuous actions (a dense representation) and the evaluator is used to evaluate these actions. More specifically; our evaluator, similar to the critic in \citet{dulac2015deep}, learns the $Q$ value for each state-action pair. \textbf{(2) Retrieval Mechanism} - We build on ideas from the sparse reconstruction literature (see \cite{elad2010book} for a survey of results). Formally, the goal is to solve $\min ||x||_0$ $\text{s.t.} \enspace Dx = v$ where $D$ is a dictionary (e.g., a matrix of word embeddings), $x$ is a sparse vector (e.g. a sentence), and $v$ is the observation (e.g. the encoder's output). There exist \textit{computationally efficient algorithms} for sparse reconstruction, under some assumptions on the structure of the dictionary (e.g., spark, coherence and RIP). \textbf{(3) Representation} - We represent words using embeddings, previously trained on a large corpus of text. Recently, \citet{arora2018compressed} demonstrated sparse reconstruction of documents from the sum of common embedding schemes such as Word2vec \citep{mikolov2013efficient} and GloVe \citep{pennington2014glove}. Similarly, we propose to reconstruct discrete actions, composed of words, from the continuous output of the encoder.

%\todo[inline]{I would swap between (2) and (3), starting with explaining the representation as embeddings and then how to retrieve the discrete action. There, consider explaining why you use CS - because the BOW representation is a sparse representation of a sentence.}

% \dis{I think you need to explain figure 1 here. It is too vague at this point. Maybe label each part of the figure with (A), (B) and (C) and then refer to these labels in the figure when discussing the World Model, Retrieval Mechanism and Representation...}

%In this work adresses this challenge explictly and We combine deep reinforcement learning with sparse recovery techniques (\cite{elad2010book} provides a good summary) in order to take advantage of this underlying structure and improve the computational efficiency.

\footnotetext[1]{Global optimality can be ensured, however the tradeoff requires a cost of $\bigO(d^l)$ during the training phase.}
\footnotetext[2]{The complexity is the sub-set of valid actions as deemed by the elimination network. In the worst case, all actions are valid and the complexity is $\bigO(d^l)$.}

% We build upon the architecture of \cite{discrete ddpg} and adapt it to our domain. We identify several difficulties which arise in the adaptation to general action spaces (i.e. text) and provide solutions.

%In this work, we focus on text-based games \citep{cote2018textworld}, in which both the states and actions are textual. Given a dictionary with $d$ entries, the number of possible sentences of length $l$ are $d^l$, hence text-based games pose an interesting and challenging task which highlights the problem of combinatorical action spaces. The novelty of our approach is an actor network which outputs a sum of word embeddings (i.e. $Dx$); we then recover $x$ (the Bag-of-Words) using a sparse reconstruction algorithm (e.g. OMP - Algorithm \ref{algo:omp}); finally, given the BoW vector, we reconstruct the most likely sentence.
%thus reducing the complexity, during inference, from $O(d^l)$ to $O(d \times l)$.
